On Bitcoin Price Prediction

In recent years, cryptocurrencies have attracted growing attention from both private investors and institutions. Among them, Bitcoin stands out for its impressive volatility and widespread influence. This paper explores the predictability of Bitcoin's price movements, drawing a parallel with traditional financial markets. We examine whether the cryptocurrency market operates under the efficient market hypothesis (EMH) or if inefficiencies still allow opportunities for arbitrage. Our methodology combines theoretical reviews, empirical analyses, machine learning approaches, and time series modeling to assess the extent to which Bitcoin's price can be predicted. We find that while, in general, the Bitcoin market tends toward efficiency, specific conditions, including information asymmetries and behavioral anomalies, occasionally create exploitable inefficiencies. However, these opportunities remain difficult to systematically identify and leverage. Our findings have implications for both investors and policymakers, particularly regarding the regulation of cryptocurrency brokers and derivatives markets.

==> Commande.tex <==
%%%%%%%%%%%%%%%     FIGURE     %%%%%%%%%%%%%%% 

\begin{figure}[!ht]
				\centering
				\includegraphics[scale=0.5, clip]{}
				\caption{}
				\label{}
\end{figure}

%%%%%%%%%%%%%%%     FIGURE     %%%%%%%%%%%%%%% 

\begin{minipage}[c]{.46\linewidth}
     gauche
\end{minipage} \hfill
\begin{minipage}[h]{.4\linewidth}
     droite
\end{minipage}

%%%%%%%%%%%%%%%     TABLEAU    %%%%%%%%%%%%%%% 

\begin{table}[h]
	\begin{center}
		\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
			\hline
			 & \\ \hline
			 & \\ \hline
		\end{tabular}
	\end{center}
	\caption{}
	\label{}
\end{table}

%%%%%%%%%%%%%%%     TABLEAU2   %%%%%%%%%%%%%%% 

\begin{table}[h]
	\begin{center}
	\begin{tabular}{|>{\columncolor[RGB]{191,191,191}}c|c|c|c|c|c|c|c|}
   \hline
   \rowcolor{lightgray} &  &  &  \\
    \hline
     &  &  & \\
    \cline{2-3} \cline{3-4}
     &  &  & \\
     \cline{2-3} \cline{3-4}
     &  &  & \\
        \hline
     &  &  & \\
    \hline
	\end{tabular}
	\end{center}
	\caption{}
    \label{}
\end{table}

%%%%%%%%%%%%%%%     EQUATION    %%%%%%%%%%%%%%

\begin{align*}
\intertext{}
            % ACCOLADES %
\left\{
      \begin{aligned}
        \\
        \\
      \end{aligned}
    \right. 
 
\numberthis
\end{align*}    

%%%%%%%%%%%%%%%     DIVERS     %%%%%%%%%%%%%%%

\renewcommand\labelitemi{\textbullet}
\hspace*{0.53cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
